Simultaneous Computation and Memory Efficient Zeroth-Order Optimizer for Fine-Tuning Large Language Models

Fine-tuning is powerful for adapting large language models to downstream tasks, but it often results in huge memory usages. A promising approach to mitigate this is using Zeroth-Order (ZO) optimization, which estimates gradients to replace First-Order (FO) gradient calculations, albeit with longer training time due to its stochastic nature. By revisiting the Memory-efficient ZO (MeZO) optimizer, we discover that the full-parameter perturbation and updating processes consume over 50% of its overall fine-tuning time cost. Based on these observations, we introduce a novel layer-wise sparse computation and memory efficient ZO optimizer, named LeZO. LeZO treats layers as fundamental units for sparsification and dynamically perturbs different parameter subsets in each step to achieve full-parameter fine-tuning. LeZO incorporates layer-wise parameter sparsity in the process of simultaneous perturbation stochastic approximation (SPSA) and ZO stochastic gradient descent (ZO-SGD). It achieves accelerated computation during perturbation and updating processes without additional memory overhead. We conduct extensive experiments with the OPT model family on the SuperGLUE benchmark and two generative tasks. The experiments show that LeZO accelerates training without compromising the performance of ZO optimization. Specifically, it achieves over 3x speedup compared to MeZO on the SST-2, BoolQ, and Copa tasks.

==> tables/speedup.tex <==
\begin{figure}[ht]
    \centering
        \begin{subfigure}{0.32\textwidth}
        \centering
          \includegraphics[width=\textwidth]{figers/opt13b-ft-sst2.pdf}
          \caption{SST-2}
      \label{fig:speedup-sst2}
      \end{subfigure}
        \begin{subfigure}{0.32\textwidth}
          \centering
          \includegraphics[width=\textwidth]{figers/opt13b-ft-boolq.pdf}
          \caption{BoolQ}
          \label{fig:speedup-boolq}
        \end{subfigure}
        \begin{subfigure}{0.32\textwidth}
          \centering
          \includegraphics[width=\textwidth]{figers/opt13b-ft-copa.pdf}
          \caption{Copa}
          \label{fig:speedup-copa}
        \end{subfigure}
    \caption{Computational speedup and convergence acceleration achieved by SSZO on three different datasets. On the classification task, SST-2, SSZO can achieve a $3.4\times$ acceleration.}
    \label{fig:speedup}
    \vspace{-16pt}
\end{figure}

==> tables/time-acc.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figers/time-dropnum-acc.pdf}
    \caption{
    % Correlation between sparsity ratio, run time on fine-tuning OPT 13b using the SSZO on the SST-2 task. 该图来自于图3中不同稀疏率下的最佳实验结果，用不同颜色的五角星进行了标注。紫色的线表示对应的实验中微调所需要的总时间。
    Correlation between the sparsity ratio and runtime on fine-tuning of OPT 13b using SSZO on the SST-2 task. This figure presents the optimal experimental results at various sparsity levels from~\Cref{fig:lr-dropnum}, annotated with different colored pentagrams. The purple line indicates the total time required for fine-tuning in the corresponding experiments.
    }
    \vspace{-10pt}
    \label{fig:time-acc}
\end{figure}
